Active TLS Stack Fingerprinting: Characterizing TLS Server Deployments at Scale

Active measurements can be used to collect server characteristics on a large scale. This kind of metadata can help discovering hidden relations and commonalities among server deployments offering new possibilities to cluster and classify them. As an example, identifying a previously-unknown cybercriminal infrastructures can be a valuable source for cyber-threat intelligence. We propose herein an active measurement-based methodology for acquiring Transport Layer Security (TLS) metadata from servers and leverage it for their fingerprinting. Our fingerprints capture the characteristic behavior of the TLS stack primarily caused by the implementation, configuration, and hardware support of the underlying server. Using an empirical optimization strategy that maximizes information gain from every handshake to minimize measurement costs, we generated 10 general-purpose Client Hellos used as scanning probes to create a large database of TLS configurations used for classifying servers. We fingerprinted 28 million servers from the Alexa and Majestic toplists and two Command and Control (C2) blocklists over a period of 30 weeks with weekly snapshots as foundation for two long-term case studies: classification of Content Delivery Network and C2 servers. The proposed methodology shows a precision of more than 99 % and enables a stable identification of new servers over time. This study describes a new opportunity for active measurements to provide valuable insights into the Internet that can be used in security-relevant use cases.

==> Makefile <==
# The grand unified latex makefile
# or
# building latex is easy

# (2016) Johannes Naab <naab@net.in.tum.de>
# Originally based on work by
# Stephan Günther <guenther@tum.de>
# Maximilian Riemensberger <riemensberger@tum.de>

# Approach for dependency tracking taken from https://github.com/shiblon/latex-makefile
# Concept for fix point iteration on input files by https://github.com/aclements/latexrun

# extension and configuration go into Makefile.conf.mk

# All hope abandon ye who enter here

VERSION = 20160524.0

# make feature flags
.SECONDARY:

.SILENT :
.SECONDEXPANSION:

# output-sync supported since 4.0, which is not in OS X
# version check from https://lists.gnu.org/archive/html/help-make/2006-04/msg00065.html
# disabling built-in rules and variables only works properly since 4.0
ifeq (4.0,$(firstword $(sort $(MAKE_VERSION) 4.0)))
	MAKEFLAGS += -r -R -Oline
endif

FIGUREDIR := figures
BUILDDIR := build
.DEFAULT_GOAL := all

CURDIRBASE := $(notdir $(CURDIR))
RELEASE_FILENAME := $(CURDIRBASE).tar.gz

PDFLATEX ?= pdflatex
BIBTEX ?= bibtex
DIFF ?= diff
GREP ?= grep
AWK ?= awk
LS ?= ls
MV ?= mv
SED ?= sed
UNIQ ?= uniq
SORT ?= sort
FIND ?= find
TAR ?= tar
OPENSSL ?= openssl
CMP ?= cmp
XARGS ?= xargs

# http://stackoverflow.com/a/12099167
UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Linux)
	TAROPTS = --no-recursion
endif
ifeq ($(UNAME_S),Darwin)
	TAROPTS = -n
endif


# terminal colors
ifneq ($(COLORTERM),false)
  NOCOLOR := "\033[0m"
  RED := "\033[1;31m"
  BLUE := "\033[1;34m"
  GREEN := "\033[1;32m"
  YELLOW := "\033[1;33m"
  CYAN := "\033[1;36m"
  WHITE := "\033[1;37m"
  MAGENTA := "\033[1;35m"
  BOLD := "\033[1m"
else
  NOCOLOR := ""
  RED := ""
  BLUE := ""
  GREEN := ""
  YELLOW := ""
  CYAN := ""
  WHITE := ""
  MAGENTA := ""
  BOLD := ""
endif

-include Makefile.conf.mk

PDFLATEX_FLAGS += -interaction=batchmode -recorder -file-line-error
GREP_FLAGS += -E -B 2 -A 3

TEXINPUTS := .:$(CURDIR):$(TEXINPUTS)
export TEXINPUTS

FIGURESTEXSRC += $(filter-out $(SKIP),$(wildcard $(FIGUREDIR)/*.tex))
FIGURESTEXPDF := $(FIGURESTEXSRC:.tex=.pdf)
FIGURESTIKZSRC += $(filter-out $(SKIP),$(wildcard $(FIGUREDIR)/*.tikz))
FIGURESTIKZPDF := $(filter-out $(FIGURESTEXPDF),$(FIGURESTIKZSRC:.tikz=.pdf))
FIGURESRC := $(FIGURESTEXSRC) $(FIGURESTIKZSRC)
FIGUREPDF := $(FIGURESTEXPDF) $(FIGURESTIKZPDF)

ALLFIGURESTIKZPDF := $(FIGURESTIKZPDF)
ALLFIGURESTEXPDF := $(FIGURESTEXPDF)

FIGURESUBDIRS := $(wildcard $(FIGUREDIR)/*/)
FIGURESUBDIRSTEMS := $(FIGURESUBDIRS:$(FIGUREDIR)/%/=%)

define template_FIGURESPDF
 FIGURESTEXSRC_$(1) += $$(filter-out $$(SKIP),$$(wildcard $$(FIGUREDIR)/$(1)/*.tex))
 FIGURESTEXPDF_$(1) := $$(FIGURESTEXSRC_$(1):.tex=.pdf)
 FIGURESTIKZSRC_$(1) += $$(filter-out $$(SKIP),$$(wildcard $$(FIGUREDIR)/$(1)/*.tikz))
 FIGURESTIKZPDF_$(1) := $$(filter-out $$(FIGURESTEXPDF_$(1)),$$(FIGURESTIKZSRC_$(1):.tikz=.pdf))
 FIGURESPDF_$(1) := $$(FIGURESTEXPDF_$(1)) $$(FIGURESTIKZPDF_$(1))
endef

$(foreach X,$(FIGURESUBDIRSTEMS),$(eval $(call template_FIGURESPDF,$(X))))
$(eval ALLFIGURESTEXPDF += $(FIGURESUBDIRSTEMS:%=$$(FIGURESTEXPDF_%)))
$(eval ALLFIGURESTIKZPDF += $(FIGURESUBDIRSTEMS:%=$$(FIGURESTIKZPDF_%)))
$(eval ALLFIGURESSRC += $(FIGURESUBDIRSTEMS:%=$(FIGURESTEXSRC_%)) $(FIGURESUBDIRSTEMS:%=$(FIGURESTIKZSRC_%)))

ALLFIGURESPDF := $(ALLFIGURESTEXPDF) $(ALLFIGURESTIKZPDF)

# studentdefs.tex itself does not build a pdf
TEXSRC := $(filter-out $(SKIP),$(wildcard *.tex))
TEXPDF := $(TEXSRC:.tex=.pdf)

# allow building protocol instead of protocol.pdf
TEXSTEM := $(TEXSRC:.tex=)

ALLTEXPDF := $(TEXPDF) $(ALLFIGURESPDF) $(SPECIALTEXPDF)

# only include (re-)buildable dependencies
DEPSMAKEINCLUDE := $(ALLTEXPDF:%=$(BUILDDIR)/%.d)
DEPSMAKEINCLUDEEXIST := $(wildcard $(DEPSMAKEINCLUDE))

DEPSMAKE  := $(filter-out $(DEPSMAKEINCLUDE),$(MAKEFILE_LIST))
DEPS      += $(DEPSMAKE)

# include dependency makefiles, but only if they exist (wildcard LIST)
# in order to force creation/update if *.d was deleted
$(DEPSMAKEINCLUDEEXIST): ;
include $(DEPSMAKEINCLUDEEXIST)

# debugging helper
# based on http://www.cmcrossroads.com/article/printing-value-makefile-variable
print-%:
	$(warning $*=$($*) ($(value $*)))

# http://www.cmcrossroads.com/article/dumping-every-makefile-variable
.PHONY: printvars
printvars:
	@$(foreach V, $(sort $(.VARIABLES)), $(if $(filter-out environment% default automatic, $(origin $V)), $(warning $V=$($V) ($(value $V)))))

# help output
# based on https://gist.github.com/rcmachado/af3db315e31383502660
.PHONY: help
help: ## Show this help
	@printf 'Usage: make [target]\n\n'
	@printf 'available targets\n'
	@awk '/^[a-zA-Z\-\_0-9]+:/ {					\
		nb = sub( /^## /, "", helpMsg );			\
		if(nb == 0) {						\
			helpMsg = $$0;					\
			nb = sub( /^[^:]*:.* ## /, "", helpMsg );	\
		}							\
		if (nb)							\
			print   $$1 "#" helpMsg;			\
	}								\
	{ helpMsg = $$0 }'						\
	$(MAKEFILE_LIST) |						\
	column -ts $$'#' |						\
	sed 's/^/\t/' |							\
	grep --color=auto '^[^ ]*'


# since empty include targets are not remade, create empty dependency includes
# https://www.gnu.org/software/make/manual/html_node/Remaking-Makefiles.html#Remaking-Makefiles
$(BUILDDIR)/%.d: MAGIC
	mkdir -p $(dir $@)
	touch $@

.PHONY: MAGIC
MAGIC:


# messaging functions
msgpdfstart = printf "building "$(BOLD)"%s"$(NOCOLOR)" from %s%s\n" "$(2)" "$(1)" "$(if $(3), -jobname=$(3))"
msgtarget = printf $(GREEN)"%s"$(MAGENTA)" %s"$(NOCOLOR)"\n" "$(1)" "$(2)"
msgcompile = printf $(BOLD)"%s"$(NOCOLOR)" %s from %s\n" "[$(1)]" "$(4)" "$(2)$(if $(3), -jobname $(3))"
msgfail = printf $(RED)"%s"$(NOCOLOR)" using %s %s "$(RED)"FAILED!"$(NOCOLOR)"\n" "$(4)" "$(1)" "$(2)$(if $(3), -jobname $(3))"

# $(1) document
# $(2) jobname
# $(3) output-directory
# $(4) target (for logging)
define run-typeset
  $(call msgcompile,$(PDFLATEX),$(1),$(2),$(4)); \
  ( cd $(3) && $(PDFLATEX) $(PDFLATEX_FLAGS) $(if $(2),-jobname=$(2)) $(1) ) </dev/null >/dev/null 2>&1 || \
    { $(call msgfail,$(PDFLATEX),$(1),$(2),$(4)); false; }
endef

# $(1) aux file
# $(2) target (for logging)
define run-bibtex
  $(call msgcompile,$(BIBTEX),$(1),,$(2)); \
  $(BIBTEX) $(BIBTEX_FLAGS) $(1) </dev/null 1>/dev/null 2>&1 || \
    { $(call msgfail,$(BIBTEX),$(1),,$(2)); false; }
endef

# $(1) log file
# $(2) target (for reference)
define extract-log
  printf "Extracting log for "$(MAGENTA)"%s"$(NOCOLOR)" from "$(GREEN)"%s"$(NOCOLOR)"\n" "$(2)" "$(1)"; \
  $(GREP) -E -v -e "^<Error-correction level increased from . to . at no cost\\.>$$" $(1) | \
  $(GREP) $(GREP_FLAGS) -e ":[[:digit:]]+: |Warning|Error|Underfull|Overfull|\!|Reference|Label|Citation" || :
endef

# $(call get-inputs,<jobname>,<target>)
# $(1) outstem
# $(2) document
define get-inputs
$(AWK) 'BEGIN { rel="$(CURDIR)"; if (rel !~ /\/$$/) {rel = rel "/"}; target="$(2)"; gsub(" ","\\\\ ",target); } \
/^PWD / {path=substr($$0,5) "/"} \
/^INPUT / { \
	f=substr($$0,7); \
	if (f ~ /^\.\//) {f=path substr(f,3)}; \
	if (f !~ /^\//) {f=path f}; \
	sub(rel,"",f); \
	if (f !~ /\%/ && f != "/dev/null") { all[f] }\
} END { for (i in all) {gsub(" ", "\\\\ ",i); print target ": " i; print i ":";} }' $(1).fls |\
sort
endef

# $(1) foo.fls
# $(2) outputdir
define check-inputs
{ echo $1.nav; echo $1.snm; echo $1.out; $(AWK) '/^INPUT / { print substr($$0,7) }' $1.fls; } | sort -u | $(XARGS) $(OPENSSL) sha512 2>/dev/null
endef

# $(1) outstem
# $(2) target
define get-bib-inputs
$(SED) -n 's!^\\bibdata{\(.*\)}$$!\1.bib!p' $(1).aux | \
$(SORT) -u | \
$(AWK) '{ print "$2: "p$$0; print p$$0":"; }'
endef

# $(1) document
# $(2) jobname
define getjobstem
$(if $(2),$(2),$(basename $(notdir $(1))))
endef

# $(1) document, required
# $(2) jobname
# $(3) builddir, if set this is used directly, else the build dir is constructed based on $(BUILDDIR), document and jobname
define getbuilddir
$(if $(3),$(3),$(BUILDDIR)/$(1)/$(call getjobstem,$(1),$(2)))
endef

# $(1) document, required
# $(2) jobname
# $(3) output
define getoutstem
$(call getbuilddir,$(1),$(2),$(3))/$(call getjobstem,$(1),$(2))
endef

# $(1) doc, required
# $(2) out, required
# $(3) jobname, can be empty
# $(4) outdir, required
# $(5) outstem, required
define pdfbuilderexpsinglepass
$(call run-typeset,$(1),$(3),$(4),$(2)) || touch $(4).error ; \
$(AWK) '/^\\bibdata{/{b=1}END{if (b) {exit 1} else {exit 0}}' $(5).aux || { $(call run-bibtex,$(5).aux,$(2)) || touch $(4).error ; } ;\
( cd $(4) && $(call check-inputs,$(notdir $(5))) ) > $(4).inputs.new ;\
cmp -s $(4).inputs.new $(4).inputs || { \
mv $(4).inputs.new $(4).inputs ;\
} ;
endef

# $(1) doc, required
# $(2) out, required
# $(3) jobname, can be empty
# $(4) outdir, required
# $(5) outstem, required
define pdfbuilderexpsinglepasstry
test -e $(4).inputs.new || { $(call pdfbuilderexpsinglepass,$(1),$(2),$(3),$(4),$(5)) } ;
endef

# $(1) doc, required
# $(2) out, required
# $(3) jobname, can be empty
# $(4) outdir, required
# $(5) outstem, required
# concept of fix point iteration taken from https://github.com/aclements/latexrun
# ideally we would set .DELETE_ON_ERROR, but this would break any preview
# so we roll our own error handling with $(4).error
define pdfbuilderexp
$(call msgpdfstart,$(1),$(2),$(3))
mkdir -p $(4)
rm -rf $(4).error
( test -e $(5).fls && cd $(4) && $(call check-inputs,$(notdir $(5))) ) > $(4).inputs || true
$(call pdfbuilderexpsinglepass,$(1),$(2),$(3),$(4),$(5))
$(call pdfbuilderexpsinglepasstry,$(1),$(2),$(3),$(4),$(5))
$(call pdfbuilderexpsinglepasstry,$(1),$(2),$(3),$(4),$(5))
$(call pdfbuilderexpsinglepasstry,$(1),$(2),$(3),$(4),$(5))
$(call pdfbuilderexpsinglepasstry,$(1),$(2),$(3),$(4),$(5))
test -e $(4).inputs.new || printf $(RED)"%s"$(NOCOLOR)": "$(BOLD)"fix point iteration failed"$(NOCOLOR)"\n" "$(2)"
$(call extract-log,$(5).log,$(2))
$(call get-inputs,$(5),$@) > $(BUILDDIR)/$@.d
$(call get-bib-inputs,$(5),$@) >> $(BUILDDIR)/$@.d
test -e $(4).error || touch -r $(BUILDDIR)/$@.d $(5).pdf
mkdir -p $(dir $(2))
$(MV) $(5).pdf $(2)
test ! -e $(4).error
endef

# $(1) doc, required
# $(2) out, required
# $(3) jobname
# $(4) builddir
define pdfbuilder
$(call pdfbuilderexp,$(1),$(2),$(3),$(call getbuilddir,$(1),$(3),$(4)),$(call getoutstem,$(1),$(3),$(4)))
endef

.PHONY: $(TEXSTEM)
$(TEXSTEM): %: %.pdf ;

# target for directly build documents without jobname
$(filter-out $(ALLFIGURESPDF),$(ALLTEXPDF)): $(FIGUREPDF)
$(filter-out $(ALLFIGURESTIKZPDF) $(SPECIALTEXPDF),$(ALLTEXPDF)): %.pdf: %.tex $$(DEPS_$$*) $$(FIGURESPDF_$$*) $(DEPS) $(BUILDDIR)/$$@.d
	$(call pdfbuilder,$<,$@)

# use hard coded for shell completion
.PHONY: $(FIGUREDIR)
$(FIGUREDIR): $(ALLFIGURESPDF)

# tikz figures, other figures are built by generic *.pdf target
$(ALLFIGURESTIKZPDF): %.pdf: %.tikz $$(DEPS_$$*) $(DEPS) $(BUILDDIR)/$$@.d
	$(call pdfbuilder,$<,$@)

.PHONY: all
all: $(ALLTEXPDF)

.PHONY : clean cleanall
clean:
	rm -fv $(DEPSMAKEINCLUDE)
	rm -rfv $(addprefix $(BUILDDIR)/,$(FIGURESRC) $(TEXSRC) $(ALLFIGURESSRC))

cleanall: clean
	rm -fv pandoc/*.tex
	rm -fv figures/*.synctex.gz
	rm -fv *.synctex.gz
	rm -fv *.nav
	rm -fv *.fls
	rm -fv *.snm
	rm -fv *.out
	rm -fv *.toc
	rm -fv *.aux
	rm -fv *.bbl
	rm -fv *.blg
	rm -fv *.log
	rm -fv figures/*.nav
	rm -fv figures/*.fls
	rm -fv figures/*.snm
	rm -fv figures/*.out
	rm -fv figures/*.toc
	rm -fv figures/*.aux
	rm -fv figures/*.log
	rm -fv $(ALLTEXPDF)
	rm -rfv $(BUILDDIR)/

.PHONY: release $(RELEASE_FILENAME)
$(RELEASE_FILENAME): cleanall
	cd .. \
		&& $(FIND) "$(CURDIRBASE)" ! -path "$(CURDIRBASE)" ! -path "$(CURDIRBASE)/$@" -print0 \
		| $(TAR) -cvzf "$(CURDIRBASE)/$@" $(TAROPTS) -h --null -T -

release: $(RELEASE_FILENAME)

